Creating high-contrast patterns in multiple-scattering media via wavefront shaping

Wavefront shaping allows focusing light through or inside strongly scattering media, but the background intensity also increases due to long-range correlations, reducing the target's contrast. By manipulating non-local intensity correlations of scattered waves in a disordered system with input wavefront shaping, we create high-contrast patterns behind strongly scattering media and targeted energy delivery into a diffusive system with minimal change in the surrounding intensity. These are achieved by introducing the contrast operator and the difference operator, and utilizing their eigenstates to maximize the target-to-background intensity contrast and energy difference. This work opens the door to coherent control of non-local effects in wave transport for practical applications.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
